Cooperative Routing for Wireless Networks using Mutual-Information Accumulation

Cooperation between the nodes of wireless multihop networks can increase communication reliability, reduce energy consumption, and decrease latency. The possible improvements are even greater when nodes perform mutual information accumulation using rateless codes. In this paper, we investigate routing problems in such networks. Given a network, a source, and a destination, our objective is to minimize end-to-end transmission delay under energy and bandwidth constraints. We provide an algorithm that determines which nodes should participate in forwarding the message and what resources (time, energy, bandwidth) should be allocated to each. Our approach factors into two sub-problems, each of which can be solved efficiently. For any transmission order we show that solving for the optimum resource allocation can be formulated as a linear programming problem. We then show that the transmission order can be improved systematically by swapping nodes based on the solution of the linear program. Solving a sequence of linear programs leads to a locally optimal solution in a very efficient manner. In comparison to the proposed cooperative routing solution, it is observed that conventional shortest path multihop routing typically incurs additional delays and energy expenditures on the order of 70%. Our first algorithm is centralized, assuming that routing computations can be done at a central processor with full access to channel state information for the entire system. We also design two distributed routing algorithms that require only local channel state information. We provide simulations showing that for the same networks the distributed algorithms find routes that are only about two to five percent less efficient than the centralized algorithm.

==> conclusions.tex <==
\section{Summary and conclusions}
\label{sec.conclusion}



In this paper we analyze the problem of generalized routing in
cooperative relay networks that use mutual-information accumulation.
We split the routing problem into one of finding the best \transOrder
and one of finding the best resource allocation given a
\transOrderNoSpace.  As our solution is based on solving a sequence of
linear programs, it is quite numerically efficient, even for large
networks.  We also show that under equal per-node PSDs, the
minimum-delay solution also minimizes energy consumption.  The
resulting route is markedly different from the conventional
shortest-path route.  The delay (and energy usage) of the latter is
about 70 \% more in the examples we present. We also develop
distributed algorithms that retain most of the performance gains
without requiring centralized knowledge of channel state information.

The approach presented in this paper is a step towards practically
realizing cooperative communications in large networks.  Future work
will focus on optimizing the power allocation (adjusting the
$\nodeP{i}$), algorithms that are suitable for imperfect channel state
information, and the impact of non-ideal codes and hardware.

{\bf Acknowledgements:} We thank Dr. Neelesh Mehta for useful
discussions, and Dr. Jin Zhang, Dr. Kent Wittenburg, and Dr. Joseph
Katz for their support and encouragement.

